Auction learning as a two-player game

Designing an incentive compatible auction that maximizes expected revenue is a central problem in Auction Design. While theoretical approaches to the problem have hit some limits, a recent research direction initiated by Duetting et al. (2019) consists in building neural network architectures to find optimal auctions. We propose two conceptual deviations from their approach which result in enhanced performance. First, we use recent results in theoretical auction design (Rubinstein and Weinberg, 2018) to introduce a time-independent Lagrangian. This not only circumvents the need for an expensive hyper-parameter search (as in prior work), but also provides a principled metric to compare the performance of two auctions (absent from prior work). Second, the optimization procedure in previous work uses an inner maximization loop to compute optimal misreports. We amortize this process through the introduction of an additional neural network. We demonstrate the effectiveness of our approach by learning competitive or strictly improved auctions compared to prior work. Both results together further imply a novel formulation of Auction Design as a two-player game with stationary utility functions.

==> ICLR Auction Game/abstract.tex <==

Designing an incentive compatible auction that maximizes expected revenue is a central problem in Auction Design. While theoretical approaches to the problem have hit some limits, a recent research direction initiated by \cite{dutting2017optimal} consists in building neural network architectures to find optimal auctions. We propose two conceptual deviations from their approach which result in enhanced performance. First, we use recent results in theoretical auction design to introduce a \emph{time-independent} Lagrangian. This not only circumvents the need for an expensive hyper-parameter search (as in prior work), but also provides a single metric to compare the performance of two auctions (absent from prior work). Second,the optimization procedure in previous work uses an inner maximization loop to compute optimal misreports.  We amortize this process through the introduction of an additional neural network. We demonstrate the effectiveness of our approach by learning competitive or strictly improved auctions compared to prior work. Both results together further imply a novel formulation of Auction Design as a two-player game with stationary utility functions.


==> ICLR Auction Game/architectures.tex <==
\vspace{-1em}
\section{Architecture and training procedure}\label{sec:NN_arch}
\vspace{-0.7em}
We describe ALGnet, a feed-forward architecture solving for the game formulation \eqref{eq:game} and then provide a training procedure. ALGnet consists in two modules that are the auctioneer's module and the misreporter's module. These components take as input a bid matrix $B = (b_{i,j})\in \mathbb{R}^{n\times m}$ and are trained jointly. Their outputs are used to compute the regret and revenue of the auction. 

\paragraph{Notation.} We use  $ \text{MLP}(d_{\text{in}},n_l,h,d_{\text{out}})$ to refer to  a fully-connected neural network  with input dimension $d_{\text{in}}$, output dimension $d_{\text{out}}$ and $n_l$ hidden layers of width $h$ and $\mathrm{tanh}$ activation function. $\mathrm{sig}$ denotes the sigmoid activation function. Given a matrix $B=[\vec{b}_1,\dots,\vec{b}_n]^{\top}\in \mathbb{R}^{n\times m},$ we define for a fixed $i\in N$, the matrix $B_{(i)}:=[\vec{b}_i,\vec{b}_1,\dots,\vec{b}_{i-1},\vec{b}_{i+1},\dots,\vec{b}_n].$ 
% Lastly, $\vec{B}\in \mathbb{R}^{nm}$ denotes the vectorization of the matrix $B$.

\subsection{The Auctioneer's module}

 It is composed of an allocation network that encodes a  randomized  allocation $g^w\colon \mathbb{R}^{nm} \to [0,1]^{nm}$ and a  payment network that encodes a payment rule $p^w\colon \mathbb{R}^{nm} \to \mathbb{R}^{n}$. 


\paragraph{Allocation network.} It computes the allocation probabily of item $j$ to bidder $i$ $[g^w(B)]_{ij}$ as $[g^w(B)]_{ij} = [f_1(B)]_j\cdot [f_2(B)]_{ij}$ where $f_1\colon \mathbb{R}^{n\times m} \to [0,1]^{m}$ and $f_2\colon\mathbb{R}^{n\times m} \to [0,1]^{m \times n }$ are functions 
computed by two feed-forward neural networks.\\
\hspace*{.2cm} -- $[f_1(B)]_j$ is the probability that object $j \in M$ is allocated and is given by ${[f_1(B)]_j = \mathrm{sig}\left(\text{MLP}(nm,n_{a},h_a,n)\right)}$. \\
\hspace*{.3cm} --\; $[f_2(B)]_{ij}$ is the probability that item $j\in M$ is allocated to bidder $i\in N$ conditioned on object $j$ being allocated. A first MLP computes  $l_j:=\text{MLP}(nm,n_{a},h_a,m)(B_{(j)})$ for all $j\in M$. The network then concatenates all these vectors $l_j$ into a matrix $L\in \mathbb{R}^{n\times m}$. A softmax activation function is finally applied to $L$ to ensure feasibility i.e. for all $j\in M, \sum_{i\in N}L_{ij} = 1.$ 


\paragraph{Payment network.}

It computes the payment $[p^w(B)]_i$ for bidder $i$ as $[p^w(B)]_i = \tilde{p}_i \sum_{j=1}^m B_{ij}[g^w(B)]_{ij},$ where $\tilde{p}\colon \mathbb{R}^{n\times m}\rightarrow [0,1]^n.$ $\tilde{p}_i$ is the fraction of bidder’s $i$ utility that she has to pay to the mechanism. We  compute $ \tilde{p}_i = \mathrm{sig}\left(\text{MLP}(nm,n_{p},h_p,1)\right)(B_{(i)}).$  Finally, 
notice that by construction $[p^w(B)]_i \leq \sum_{j=1}^m B_{ij}g^w(B)_{ij}$ which ensures that \eqref{eq:IR_eq} is respected.


\subsection{The Misreporter's module}
The module consists in an $\text{MLP}(nm,n_{M},h_M,m)$ followed by a projection layer $\mathrm{Proj}$ that ensure that the output of the network is in the domain $D$ of the valuation.  For example when the valuations are restricted to $[0,1]$, we can take $\mathrm{Proj=sig},$ if they are non negative number,we can take $\mathrm{Proj=SoftPlus}$. The optimal misreport for bidder $i$ is then given by $\text{Proj} \circ \text{MLP}(nm,n_{M},h_M,m)(B_{(i)}) \in \mathbb{R}^m$. Stacking these vectors gives us the misreport matrix $M^{\phi}(B)$.



\subsection{Training procedure and optimization}
\begin{minipage}[t]{0.45\linewidth}
We optimize the game \eqref{eq:game} over the space of  neural networks parameters $(w,\varphi).$ The algorithm is easy to implement (\autoref{alg:gameAlgorithm}).





 At each time $t$, we sample a batch of valuation profiles of size $B$.  The algorithm performs $\tau$ updates for the Misreporter's network (line 9) and one update on the Auctioneer's network (line 10). Moreover, we often reinitialize the Misreporter's network every $T_{init}$ steps in the early phases of the training ($t\leq T_{limit}$). This step is not necessary but we found empirically that it speeds up training. 

 \end{minipage}
 \hspace*{.3cm}
\begin{minipage}[t]{.52\textwidth}

\vspace*{-.6cm}

\begin{algorithm}[H]
\caption{ALGnet training} 
\label{alg:gameAlgorithm}
\begin{algorithmic}[1]
%\State Initialization:
\State \textbf{Input}: number of agents, number of objects.
\State \textbf{Parameter}: $\gamma >0 ;\; B, T, T_{init},  T_{limit}, \tau \in \mathbb{N}.$
\State \textbf{Initialize} misreport's and auctioneer's nets.
%\State Main routine:
\For {$t=1,\dots,T$}
    \If{$t \equiv 0\; \mathrm{mod}\;  T_{init}$ and $t < T_{Limit}$}:\\
      \hspace{1cm}  Reinitialize Misreport Network
        \EndIf
\State Sample valuation batch $S$ of size $B$.
\For{$s=1,\dots,\tau$}
    \State \hspace{-.2cm}\mbox{ $\phi^{s+1}\leftarrow \phi^{s}-\gamma \nabla_\phi \mathcal{L}_{r}(\phi^{s},w^t)(S). $}
    \EndFor
\State \mbox{\hspace{-.1cm} $w^{t+1}\leftarrow w^t-\gamma \nabla_w \mathcal{L}_{m}(w^t,\phi)(S). $}
\EndFor
\end{algorithmic}
\end{algorithm}

\end{minipage}

\vspace{-4mm}

==> ICLR Auction Game/commands.tex <==
%% Symboles avec double lignes
\newcommand{\NN}{\mathbb{N}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\PP}{\mathbb{P}}
\renewcommand{\SS}{\mathbb{S}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
%% Symboles arrondis
\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dd}{\mathcal{D}}
\newcommand{\Ee}{\mathcal{E}}
\newcommand{\Ff}{\mathcal{F}}
\newcommand{\Gg}{\mathcal{G}}
\newcommand{\Hh}{\mathcal{H}}
\newcommand{\Ii}{\mathcal{I}}
\newcommand{\Jj}{\mathcal{J}}
\newcommand{\Kk}{\mathcal{K}}
\newcommand{\Ll}{\mathcal{L}}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Oo}{\mathcal{O}}
\newcommand{\Pp}{\mathcal{P}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\Rr}{\mathcal{R}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Tt}{\mathcal{T}}
\newcommand{\Uu}{\mathcal{U}}
\newcommand{\Vv}{\mathcal{V}}
\newcommand{\Ww}{\mathcal{W}}
\newcommand{\Xx}{\mathcal{X}}
\newcommand{\Yy}{\mathcal{Y}}
\newcommand{\Zz}{\mathcal{Z}}
 

\makeatletter
\newcommand{\leqnomode}{\tagsleft@true\let\veqno\@@leqno}
\makeatother 
 
% matrices
\newcommand{\A}{\bm{A}}
\newcommand{\B}{\bm{B}}
% \newcommand{\C}{\bm{C}}
\newcommand{\D}{\bm{D}}
%\newcommand{\E}{\bm{E}}
\newcommand{\F}{\bm{F}}
% \newcommand{\G}{\bm{G}}
\newcommand{\Hz}{\bm{H}}
\newcommand{\I}{\bm{I}}
\newcommand{\J}{\bm{J}}
\newcommand{\K}{\bm{K}}
\newcommand{\Lz}{\bm{L}}
\newcommand{\M}{\bm{M}}
\newcommand{\N}{\bm{N}}
\newcommand{\Oz}{\bm{O}}
\newcommand{\Pz}{\bm{P}}
\newcommand{\Q}{\bm{Q}}
\newcommand{\R}{\bm{R}}
\newcommand{\Sz}{\bm{S}}
\newcommand{\T}{\bm{T}}
% \newcommand{\U}{\bm{U}}
\newcommand{\V}{\bm{V}}
\newcommand{\W}{\bm{W}}
\newcommand{\X}{\bm{X}}
\newcommand{\Y}{\bm{Y}}
\newcommand{\Z}{\bm{Z}}

% Vectors
\renewcommand{\a}{\bm{a}}
\renewcommand{\b}{\bm{b}}
\renewcommand{\c}{\bm{c}}
\renewcommand{\d}{\bm{d}}
\newcommand{\e}{\bm{e}}
% \newcommand{\f}{\bm{f}}
\newcommand{\g}{\bm{g}}
\newcommand{\h}{\bm{h}}
\renewcommand{\i}{\bm{i}}
\renewcommand{\j}{\bm{j}}
\renewcommand{\k}{\bm{k}}
\renewcommand{\l}{\bm{l}}
\newcommand{\m}{\bm{m}}
\newcommand{\n}{\bm{n}}
\renewcommand{\o}{\bm{o}}
\newcommand{\p}{\bm{p}}
\newcommand{\q}{\bm{q}}
\renewcommand{\r}{\bm{r}}
\newcommand{\s}{\bm{s}}
\renewcommand{\t}{\bm{t}}
\renewcommand{\u}{\bm{u}}
\renewcommand{\v}{\bm{v}}
\newcommand{\w}{\bm{w}}
\newcommand{\x}{\bm{x}}
\newcommand{\y}{\bm{y}}
\newcommand{\z}{\bm{z}}

% greek
\newcommand{\al}{\alpha}
\newcommand{\la}{\lambda}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\La}{\Lambda}
\newcommand{\si}{\sigma}
%\newcommand{\Si}{\Sigma}
\newcommand{\be}{\beta}
\newcommand{\de}{\delta}
\newcommand{\De}{\Delta}
\renewcommand{\phi}{\varphi}
\renewcommand{\th}{\theta}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}

% hat, tilde
\newcommand{\hf}{\hat f}
\newcommand{\wtf}{\tilde f}
\newcommand{\tx}{\tilde x}
\newcommand{\ta}{\tilde a}
\newcommand{\tb}{\tilde b}
\newcommand{\ty}{\tilde y}
\newcommand{\tu}{\tilde u}
\newcommand{\tv}{\tilde v}
\newcommand{\tga}{\tilde \ga}
\newcommand{\tf}{\wt{f}}

 

\newcommand{\Simplex}{\triangle}
\newcommand{\errnash}{\text{Err}_N}

% full, alternate, random
\newcommand{\full}{\textnormal{full}}
\newcommand{\cyc}{\textnormal{cyc}}
\newcommand{\rdm}{\textnormal{rand}}

%%%%%%%%%%%%%%% MATHS OPERATORS %%%%%%%%%%%%%%%%%
\newcommand{\ins}[1]{\mathrm{#1}}

\DeclareMathOperator{\realp}{\Rr e}
\DeclareMathOperator{\imagp}{\Ii m}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Supp}{Supp}
\DeclareMathOperator{\Sign}{Sign}
\let\Im\relax
\DeclareMathOperator{\Im}{Im}
% \let\span\relax
%\DeclareMathOperator{\span}{span}
\DeclareMathOperator{\Corr}{Corr}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\supp}{supp}

\DeclareMathOperator{\cas}{cas}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\Card}{Card}
\DeclareMathOperator{\GCD}{GCD}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\interop}{int}

\newcommand{\ps}[2]{\langle #1,#2\rangle}
\newcommand{\E}[1]{\mathbb{E}\left[#1\right] }

% regularity
\newcommand{\Calpha}{\mathrm{C}^\al}
\newcommand{\Cbeta}{\mathrm{C}^\be}
\newcommand{\Cal}{\text{C}^\al}
\newcommand{\Ctwo}{\text{C}^{2}}
\newcommand{\Calt}[1]{\text{C}^{#1}}
\newcommand{\Cder}[1]{\mathscr{C}^{#1}}
% Lp spaces
\newcommand{\lone}{\ell^1}
\newcommand{\ltwo}{\ell^2}
\newcommand{\linf}{\ell^\infty}
\newcommand{\Lone}{\text{\upshape L}^1}
\newcommand{\Ltwo}{\text{\upshape L}^2}
\newcommand{\Linf}{\text{\upshape L}^\infty}
\newcommand{\lzero}{\ell^0}
\newcommand{\lp}{\ell^p}
% circle
\newcommand{\Sun}{\text{S}^1}
% little space after forall
\newcommand{\foralls}{\forall \,}
%% for derivatives
\newcommand{\dd}{\ins{d}}
%% Use french comparaison operator
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}


%%%%%%%%%%%%%%% MATHS CONSTRUCTS %%%%%%%%%%%%%%%

%% over-symbols
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\whwh}[1]{\hat{\hat{#1}}}
\newcommand{\wt}[1]{\widetilde{#1}}
%% partial derivatives
\newcommand{\pd}[2]{ \frac{ \partial #1}{\partial #2} }
\newcommand{\pdd}[2]{ \frac{ \partial^2 #1}{\partial #2^2} }
%% nice epsilon
\renewcommand{\epsilon}{\varepsilon}
%% Pour avoir un joli i pour les complexes
\renewcommand{\imath}{\mathrm{i}}
\newcommand{\interior}[1]{\ensuremath{\overset{\circ}{#1}}}

%% Legendre symbol
\newcommand{\legsymb}[2]{ \genfrac{(}{)}{}{}{#1}{#2} }
%% exposant pour les ordinaux
\newcommand{\ordin}[2]{ ${#1}^{ \text{#2} }$ }
%% Dot product and cross product
% \newcommand{\dotp}[2]{ \left\langle #1,\,#2 \right\rangle }
\newcommand{\dotp}[2]{\langle #1,\,#2\rangle}
\newcommand{\dotps}[2]{\langle #1,\,#2\rangle}
\newcommand{\crossp}[2]{ #1 \hat #2 }
\newcommand{\seg}[2]{\llbracket #1,\,#2 \rrbracket}
\newcommand{\brac}[1]{\left[#1\right]}
%\newcommand{\norm}[1]{|\!| #1 |\!|}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\snorm}[1]{\| #1 \|}
\newcommand{\normb}[1]{\Big|\!\Big| #1 \Big |\!\Big|}
\newcommand{\normB}[1]{\left|\!\left| #1 \right|\!\right|}
\DeclareMathOperator{\diverg}{div}
\DeclareMathOperator{\Prox}{Prox}
\newcommand{\normT}[1]{\norm{#1}_{\text{T}}}
\newcommand{\normu}[1]{\norm{#1}_{1}}
\newcommand{\normi}[1]{\norm{#1}_{\infty}}
\newcommand{\normd}[1]{\norm{#1}_{2}}
\newcommand{\normz}[1]{\norm{#1}_{0}}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert} % modified by Vincent
\newcommand{\absb}[1]{\Big| #1 \Big|}

%% Function definition
\newcommand{\func}[4]{ {\left\{  \begin{array}{ccc} #1 & \longrightarrow & #2 \\ #3 & \longmapsto & #4 \end{array}  \right.} }
% transpose
\newcommand{\transp}[1]{ {#1}^{\ins{T}} }
% l'identit�
\newcommand{\Id}{\ins{Id}}
% egal par d�finition
\newcommand{\eqdef}{\triangleq}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\interi}{int}
% \DeclareMathOperator*{\sup}{sup}

\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\newcommand*\red{\color{red}}
\newcommand{\vardbtilde}[1]{\tilde{\raisebox{0pt}[0.85\height]{$\tilde{#1}$}}}
\usepackage{accents}
\newcommand{\dbtilde}[1]{\accentset{\approx}{#1}}

%% parenthesis
\newcommand{\pa}[1]{\left( #1 \right)}
\newcommand{\bpa}[1]{\big( #1 \big)}
\newcommand{\choice}[1]{ %
	\left\{ %
		\begin{array}{l} #1 \end{array} %
	\right. }
% ensembles
\newcommand{\set}[1]{ \{ #1 \} }
\newcommand{\condset}[2]{ \left\{ #1 \;;\; #2 \right\} }


%%%%%%%%%%%%%%% SPACES %%%%%%%%%%%%%%%%%
\newcommand{\qandq}{ \quad \text{and} \quad }
\newcommand{\qqandqq}{ \qquad \text{and} \qquad }
\newcommand{\qifq}{ \quad \text{if} \quad }
\newcommand{\qqifqq}{ \qquad \text{if} \qquad }
\newcommand{\qwhereq}{ \quad \text{where} \quad }
\newcommand{\qqwhereqq}{ \qquad \text{where} \qquad }
\newcommand{\qwithq}{ \quad \text{with} \quad }
\newcommand{\qqwithqq}{ \qquad \text{with} \qquad }
\newcommand{\qforq}{ \quad \text{for} \quad }
\newcommand{\qqforqq}{ \qquad \text{for} \qquad }
\newcommand{\qqsinceqq}{ \qquad \text{since} \qquad }
\newcommand{\qsinceq}{ \quad \text{since} \quad }
\newcommand{\qarrq}{\quad\Longrightarrow\quad}
\newcommand{\qqarrqq}{\quad\Longrightarrow\quad}
\newcommand{\qiffq}{\quad\Longleftrightarrow\quad}
\newcommand{\qqiffqq}{\qquad\Longleftrightarrow\qquad}
\newcommand{\qsubjq}{ \quad \text{subject to} \quad }
\newcommand{\qqsubjqq}{ \qquad \text{subject to} \qquad }
\newcommand{\qobjq}[1]{\quad \text{#1} \quad}
\newcommand{\qqobjqq}[1]{\quad \text{#1} \quad}

\newcommand{\carles}[1]{{\color{orange}[CD: #1]}}
\newcommand{\arthur}[1]{{\color{blue}[AM: #1]}}
\newcommand{\joan}[1]{{\color{green}[JB: #1]}}
\newcommand{\samy}[1]{{\color{red}[SJ: #1]}}


% Restrictions
% Exemple: $ \rest{f}{ \Z } $

\newlength{\restsubwidth}
\newlength{\restsubheight}
\newlength{\restsubmoreheight}
\setlength{\restsubmoreheight}{4pt}
\newcommand{\rest}[2]{%
        \settowidth{\restsubwidth}{\ensuremath{#2}}
        \settoheight{\restsubheight}{\ensuremath{{}_{#2}}}
        \ensuremath{{#1\hskip 0.5pt}_{\vrule\kern2pt\parbox[b][%
        4pt][b]{\the\restsubwidth}{%
                        \ensuremath{{}_{#2}}}}}
        }

==> ICLR Auction Game/conclusion.tex <==

\section{Conclusion}

We identified two inefficiencies in previous approaches to deep auction design and propose solutions, building upon recent trends and results from machine learning (amortization) and theoretical auction design (stationary Lagrangian). This resulted in a novel formulation of auction learning as a two-player game between an Auctioneer and a Misreporter and a new architecture ALGnet. ALGnet requires significantly fewer hyperparameters than previous Lagrangian approaches. We demonstrated the effectiveness of ALGnet on a variety of examples by comparing it to the theoretical optimal auction when it is known, and to RegretNet when the optimal solution is not known. 

{\bf Acknowledgements.} Jad Rahme would like to thank Ryan P. Adams for helpful discussions and feedback on the manuscript. Samy Jelassi thanks Arthur Mensch for fruitful discussions on the subject and feedback on the manuscript. The work of Jad Rahme was funded by a Princeton SEAS Innovation Grant. The work of Samy Jelassi is supported by the NSF CAREER CIF 1845360. The work of S. Matthew Weinberg was supported by NSF CCF-1717899.
 

==> ICLR Auction Game/criticism_dutting.tex <==

\section{Auction learning as a two-player game}\label{sec:dutt}



We first present the optimization and the training procedures for \eqref{eq:empirical_prob} proposed by \cite{dutting2017optimal}. We then demonstrate with numerical evidence that this approach presents two limitations: hyperparameter sensitivity and lack of interpretability. Using the concept of $\varepsilon$-truthful to truthful reductions, we construct a new loss function that circumvents these two aspects. Lastly, we resort to amortized optimization and reframe the auction learning problem as a two-player game.

 \subsection{The augmented Lagrangian method and its shortcomings}\label{subsec:dutt}

\paragraph{Optimization and training.} We briefly review the training procedure proposed by \cite{dutting2017optimal} to learn optimal auctions. The authors apply the augmented Lagrangian method to solve the constrained problem  \eqref{eq:empirical_prob} and consider the loss:\\ 
\vspace*{-.32cm}
\begin{equation*}
\begin{aligned}
    \mathcal{L}(w;\lambda; \rho)=-\frac{1}{L}\sum_{\ell=1}^L \sum_{i\in N} p_i^w(V^{(\ell)})+\sum_{i\in N}\lambda_i r_i^w(V^{(\ell)})+\frac{\rho}{2}\sum_{i \in N}\left(r_i^w(V^{(\ell)})\right)^2, 
\end{aligned}
\end{equation*}
where $\lambda \in\mathbb{R}^n$ is a vector of Lagrange multipliers and $\rho>0$ is a parameter controlling the weight of the quadratic penalty. More details about the training procedure can be found in Appendix A.


\paragraph{Scheduling consistency problem.} The parameters $\lambda$ and $\rho$ are time-varying. Indeed, their value changes according to a pre-defined scheduling of the following form: 1) Initialize $\lambda$ and $\rho$ with respectively   $\lambda^0$ and $\rho^0$,
2)  Update $\rho$ every $T_{\rho}$ iterations : $\rho^{t+1} \leftarrow \rho^{t} + c ,$  where $c$ is a pre-defined constant,
3) Update $\lambda$ every $T_{\lambda}$ iterations according to $\lambda_i^t \leftarrow \lambda_i^t + \rho^t \, \widehat{r}_i^{w^{t}} $.


Therefore, this scheduling requires to set up five hyper parameters $(\lambda^0,\rho^0,c,T_{\lambda},T_{\rho})$. Some of the experiments found \cite{dutting2017optimal} were about learning an optimal mechanism for an $n $-bidder $m$-item auction ($n \times m$) where the valuations are iid $\mathcal{U}[0,1]$. Different scheduling parameters were used for different values of $n$ and $m$.  We report the values of the hyper parameters used for the $1 \times 2$, $3 \times 10$ and $5 \times 10$ settings in \autoref{tab:scheduling}(a). A natural question is whether the choice of parameters heavily affects the performance. We proceed to a numerical investigation of this questions by trying different schedulings (columns) for different settings (rows) and report our the results in \autoref{tab:scheduling}(b).

\begin{table}[H]
\caption{(a): Scheduling parameters values set in \cite{dutting2017optimal} to reach optimal auctions in $n\times m$ settings with $n$ bidders, $m$ objects and i.i.d. valuations sampled from $\mathcal{U}[0,1].$ (b): Revenue $\mathit{rev}:=\mathbb{E}_{V\sim D}[\sum_{i=1}^n p_i(V)]$ and average regret per bidder $\mathit{reg}:= \nicefrac{1}{n} \, \mathbb{E}_{V \in D}\left[\sum_{i=1}^n r_i(V)\right] $ for $n\times m$ settings when using the different parameters values set reported in (a). }\label{tab:scheduling}  
\begin{minipage}{0.3\textwidth}
{\hspace{-.0cm}\resizebox{0.95\columnwidth}{!}{ 
\begin{tabular}{lccc}
\toprule
\multirow{1}{*}{ } & 
\multicolumn{1}{c}{ $1 \times 2$} & \multicolumn{1}{c}{ $3 \times 10$} & \multicolumn{1}{c}{ $5 \times 10$}
\\
\midrule
$\lambda^0$ & 5 & 5 & 1 \\
% \midrule
$\rho^0 $ & 1 & 1 & 0.25 \\
% \midrule
c & 50 & 1 & 0.25 \\
% \midrule
$T_{\lambda}$ & $10^2$ & $10^2$ & $10^2$ \\
% \midrule
$T_{\rho}$ & $10^4$ & $10^4$ & $10^5$ \\
\bottomrule
\end{tabular}}}
            \caption*{(a) }%Scheduling Parameters.
\end{minipage}
%\hfillx
\begin{minipage}{0.7\textwidth}

{\resizebox{0.95\columnwidth}{!}{ \begin{tabular}{lccccccccc}
\toprule
% \multirow{2}{*}{\diagbox[width=7.2em]{Setting}{~~Schedule}} 
\multicolumn{1}{c}{ }
& \multicolumn{6}{c}{ Scheduling} \\
\cmidrule(lr){2-7}
\multicolumn{1}{c}{}
& \multicolumn{2}{c}{ $1 \times 2$} & \multicolumn{2}{c}{ $3 \times 10$} & \multicolumn{2}{c}{ $5 \times 10$}
\\
% \cline{2-7}
    % \midrule
 \cmidrule(r){2-3}
  \cmidrule(r){4-5}
  \cmidrule(r){6-7}
Setting & $\mathit{rev}$ & $\mathit{rgt}$ & $\mathit{rev}$ & $\mathit{rgt}$ & $\mathit{rev}$ & $\mathit{rgt}$
%
\\
\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-5}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}

% \hline
 $1 \times 2$
& 0.552 & 
 0.0001 & 0.573 & 0.0012 & 0.332 & 0.0179
\\
% \hline

 $3 \times 10$  
& 4.825 & 0.0007 & 5.527 & 0.0017 & 5.880 & 0.0047 
\\
% \hline

 $5 \times 10$ 
& 4.768 & 0.0006 & 5.424 & 0.0033 & 6.749 & 0.0047 
\\
\bottomrule

\end{tabular}}}

\caption*{(b)}%Revenue and Regret for different Schedules
        \end{minipage}
\end{table}


The auction returned by the network dramatically varies with the choice of scheduling parameters. When applying the  parameters of $1\times 2$ to $5\times 10$, we obtain a revenue that is lower by 30\%! The performance of the learning algorithm strongly depends on the specific values of the hyperparameters. Finding an adequate scheduling requires an extensive and time consuming hyperparameter search.


\paragraph{Lack of interpretability.} 

How should one compare two mechanisms with different expected revenue and regret? Is a mechanism $M_1$ with revenue $P_1 = 1.01$ and an average total regret $R_1 = 0.02$ better than a mechanism $M_2$ with $P_2 = 1.0$ and $R_2 = 0.01$ ?  The approach in \cite{dutting2017optimal} cannot answer this question. To see that, notice that when $\lambda_1 = \cdots = \lambda_n =\lambda$  we can rewrite ${\mathcal{L}(w;\lambda; \rho) = - P + \lambda R + \frac{\rho}{2} R^2}$. Which mechanism is better depends on the values of $\lambda$ and $\rho$. For example if $\rho=1$ and $\lambda =0.1$ we find that $M_1$ is better, but if $\rho=1$ and $\lambda =10$ then $M_2$ is better. Since the values of $\lambda$ and $\rho$ change with time, the Lagrangian approach in \cite{dutting2017optimal} cannot provide metric to compare two mechanisms.




\subsection{A time-independent and interpretable loss function for auction learning}\label{sec:new_loss}
\vspace{-0.5em}
Our first contribution consists in introducing a new loss function for auction learning that addresses the two first limitations of \cite{dutting2017optimal} mentioned in Section~ \ref{subsec:dutt}. We first motivate this loss in the one bidder case and then extend it to auctions with many bidders.



\subsubsection{Mechanisms with one bidder}
\label{subsection:onebidder}

\begin{proposition}
\label{prop:main}[\cite{BalcanBHY05}, attributed to Nisan]
Let $\mathcal{M}$ be an additive auction with $1$~bidder and $m$~items. Let $P$ and $R$  denote the expected revenue and regret, $P  = \mathbb{E}_{V \in D}\left[ p(V) \right]$ and $R = \mathbb{E}_{V \in D}\left[ r(V)\right]$.
There exists a mechanism $\mathcal{M}^{*}$ with expected revenue $P^{*} = (\sqrt{P }-\sqrt{R })^2$ and zero regret $R^{*} = 0$.
\end{proposition}

A proof of this proposition can be found in Appendix C. Comparing two mechanisms is straightforward when both of them have zero-regret: the best one achieves the highest revenue. \autoref{prop:main} allows a natural and simple extension of this criteria for non zero-regret mechanism with one bidder: { we will say that $M_1$ is better than $M_2$ if and only if $M_1^{*}$ is better than $M_2^{*}$:}

\begin{equation}
    M_1 \geq M_2 \iff P^{*}(M_1) \geq P^{*}(M_2) \iff \sqrt{P_1}-\sqrt{R_1}  \geq \sqrt{P_2}-\sqrt{R_2}
\end{equation}
{ Using our metric, we find that a one bidder mechanism with revenue of $1.00$ and regret of $0.01$ is ''better'' than one with revenue $1.01$ and regret $0.02$.}


\subsubsection{Mechanisms with multiple bidders}

Let $M_1$ and $M_2$ be two mechanisms with $n$ bidders and $m$ objects. Let $P_i$ and $R_i$  denote their total expected revenue and regret, $P_i  = \mathbb{E}_{V \in D}\left[ \sum_{j=1}^n p_j(V) \right]$ and $R_i = \mathbb{E}_{V \in D}\left[\sum_{j=1}^n r_j(V)\right]$. {We can extend  our metric}  derived in Section~\ref{subsection:onebidder} to the multiple bidder by the following: 

\begin{equation}
  M_1 \text{ is ''better'' than } M_2 \iff   M_1 \geq M_2 \iff  \sqrt{P_1}-\sqrt{R_1}  \geq \sqrt{P_2}-\sqrt{R_2}
\end{equation}
When $n=1$ we recover the criteria from Section~\ref{subsection:onebidder} that is backed by \autoref{prop:main}. When $n > 1$, it is considered a major open problem whether the extension of \autoref{prop:main} still holds. Note that a multi-bidder variant of \autoref{prop:main} \emph{does} hold under a different solution concept termed ``Bayesian Incentive Compatible''~\citep{rubinstein2018simple,CaiOVZ19}, supporting the conjecture that \autoref{prop:main} indeed extends.\footnote{An auction is \emph{Bayesian Incentive Compatible} if every bidder maximizes their expected utility by truthful reporting \emph{in expectation over the other bidders' truthful bids}. Compare this to Dominant Strategy Incentive Compatible (our paper), where every bidder maximizes their expected utility by truthful reporting \emph{for all realizations of the other bidders' bids.}} Independently of whether or not \autoref{prop:main} holds, this reasoning implies a candidate loss function for the multi-bidder setting which we can evaluate empirically.

This way of comparing mechanisms motivates the use of loss function: $\mathcal{L}(P,R) = - (\sqrt{P}-\sqrt{R})$ instead of the Lagrangian from Section~\ref{sec:dutt}, and indeed this loss function works well in practice. We empirically find the loss function $\mathcal{L}_{m}(P,R) = -(\sqrt{P}-\sqrt{R}) + R$ further accelerates training, as it further (slightly) biases towards mechanisms with low regret. Both of these loss function are time-independent and hyperparameter-free.



\subsection{Amortized misreport optimization}\label{sec:amort}

To compute the regret $r_i^w(V)$ one has to solve the optimization problem:  $\max_{\vec{v}_i\hspace{.02cm}'\in \mathbb{R}^m} u_i^w(\vec{v}_i,(\vec{v}_i\hspace{.02cm}',V_{-i})) - u_i^w(\vec{v}_i,(\vec{v}_i,V_{-i}))$.  In \cite{dutting2017optimal}, this optimization problem is solved with an inner optimization loop for each valuation profile. In other words, computing the regret of each valuation profile is solved separately and independently, from scratch. 

If two valuation profiles are very close to each other, one should expect that the resulting optimization problems to have close results. We leverage this to improve training efficiency.

We propose to amortize this inner loop optimization. Instead of solving all these optimization problems independently, we will instead learn one neural network $M^{\phi}$ that tries to predict the solution of all of them. $M^{\phi}$ takes as entry a valuation profile and maps it to the optimal misreport:
\begin{equation}
M^{\phi}:
\begin{cases}
\mathbb{R}^{n \times m} & \to \mathbb{R}^{n \times m}\\ 
V =\left[\vec{v_i}\right]_{i \in N} & \to \left[ \mbox{argmax}_{\vec{v}' \in D} u_i(\vec{v_i},(\vec{v}',V_{-i}))\right]_{i \in N}
\end{cases}
\end{equation}
The loss $\mathcal{L}_{r}$ that $M^{\phi}$ is trying to minimize follows naturally from that definition and is then given by: $
\mathcal{L}_{r}(\phi,w) = - \mathbb{E}_{V \in D} \left[\sum_{i=1}^n u^w_i(\vec{v_i},([M^{\phi}(V)]_i,V_{-i})) \right].$


\subsection{Auction learning as a two-player game}

  In this section, we combine the ideas from Sections~\ref{sec:new_loss} and \ref{sec:amort} to obtain a new formulation for the auction learning problem as a two-player game between an Auctioneer with parameter $w$ and a Misreporter with parameter $\varphi$. The optimal parameters for the auction learning problem $(w^{*},\varphi^{*})$ are a Nash Equilibrium for this game.
  
  The Auctioneer is trying to design a truthful \eqref{eq:regretDSIC} and rational \eqref{eq:IR_eq} auction that maximizes revenue. The Misreporter is trying to maximize the bidders' utility, for the current auction selected by Auctioneer, $w$. This is achieved by minimizing the loss function $\mathcal{L}_{r}(\phi,w)$ wrt to $\phi$ (as discussed in Sec~\ref{sec:amort}). The Auctioneer in turn maximizes expected revenue, for the current misreports as chosen by Misreporter. This is achieved by minimizing $\mathcal{L}_{m}(w,\varphi) = -(\sqrt{P^{w}}+\sqrt{R^{w,\varphi}}) + R^{w,\varphi}$  with respect to $w$ (as discussed in Sec~\ref{sec:new_loss}). Here, $R^{w,\varphi}$ is an estimate of the total regret that auctioneer computes for the current Misreporter $\varphi$, 
  $R^{w,\varphi} = \frac{1}{L}\sum_{\ell=1}^L \sum_{i\in N}\left(u_i^w(\vec{v}_i,([M^{\phi}(V)]_i ,V_{-i}))- u_i^w(\vec{v}_i,(\vec{v}_i,V_{-i}))\right).$ This game formulation can be summarized as follows:\\
\vspace{-0.2em}
\begin{minipage}[t]{0.40\textwidth}
\begin{align}
\label{eq:game}\tag{G} 
\begin{cases}
\hspace{-1em}
\begin{aligned}
  \text{Misreporter: } \begin{cases}
    \textbf{loss: } \mathcal{L}_r(\varphi,w) \\
    \textbf{parameter: }\varphi
    \end{cases}  
    %\min_{\varphi} \mathcal{L}_r(R(w,\varphi))
\\\\
    \quad \text{Auctioneer: } 
    %\min_{w} \mathcal{L}_m(P(w),R(w,\varphi))
    \begin{cases}
    \textbf{loss: } \mathcal{L}_m(w,\varphi) \\
    \textbf{parameter: } w 
    \end{cases}
\end{aligned}
\end{cases}
\end{align}
\end{minipage}
\hspace{2em}
\begin{minipage}[t]{0.55\textwidth}

  \centering\raisebox{\dimexpr \topskip-\height}{%
  \includegraphics[width=\textwidth]{images/diagramm.png}}
  \label{fig1}
\end{minipage}\hfill  \\
\begin{remark}
 The game formulation \eqref{eq:game} reminds us of Generative Adversarial Networks \citep{goodfellow2014generative}. Contrary to GANs, it is not a zero-sum game. 
\end{remark}

==> ICLR Auction Game/experiments.tex <==

\section{Experimental Results}\label{sec:exps}

We show that ALGnet  can  recover  near-optimal  auctions for settings where  the  optimal  solution  is known and that it  can find new auctions for settings where analytical solution are not known. Since RegretNet is already capable of discovering near optimal auctions, one cannot expect ALGnet to achieve significantly higher optimal revenue than RegretNet. The results obtained are competitive or better than the ones obtained in \cite{dutting2017optimal} while requiring much less hyperparameters (Section~\ref{sec:dutt}). 

We also evaluate ALGnet in online auctions and compare it to RegretNet. 


For each experiment, we compute the total revenue $\mathit{rev}:=\mathbb{E}_{V\sim D}[\sum_{i\in N} p_i^{w}(V)]$ and average regret $\mathit{rgt}:=\nicefrac{1}{n}\,\mathbb{E}_{V\sim D}[\sum_{i\in N} r_i^{w}(V)]$ on a test set of $10,000$ valuation profiles. We run each experiment 5 times with different random seeds and report the average and standard deviation of these runs. In our comparisons we make sure that ALGnet and RegretNet have similar sizes for  fairness (Appendix~D).



\subsection{Auctions with known and unknown optima}

\paragraph{Known settings. } We show that ALGnet is capable of recovering near optimal auction in different well-studied auctions that have an analytical solution. These are one bidder and two items auctions where the valuations of the two items $v_1$ and $v_2$ are independent. We consider the following settings.  (A): $v_1$ and $v_2$ are  i.i.d. from  $\mathcal{U}[0,1]$,  (B): $v_1 \sim \mathcal{U}[4,16]$ and $v_2\sim \mathcal{U}[4,7]$, (C): $v_1$ has density $f_1(x)=5/(1+x)^6$ and $v_2$ has density $f_2(y)=6/(1+y)^7.$ 


(A) is the celebrated Manelli-Vincent auction \citep{manelli2006bundling}; (B) is a non-i.i.d. auction and (C) is a non-i.i.d. heavy-tail auction and both of them are studied in \citet{daskalakis2017strong}. We compare our results to the theoretical optimal auction (\autoref{fig:table_small_auct}). (\citet{dutting2017optimal} does not evaluate RegretNet on settings (B) \& (C)).   During the training process, $\mathit{reg}$ decreases to 0 while  $\mathit{rev}$ and $P^{*}$ converge to the optimal revenue.  For (A), we also plot $\mathit{rev}$, $\mathit{rgt}$ and $P^{*}$ as function of the number of epochs and we compare it to RegretNet (\autoref{fig:comparaisonRegretNet}). 



\begin{minipage}[h]{0.36\linewidth}

 Contrary to ALGnet, we observe that RegretNet overestimates the revenue in the early stages of training at the expense of a higher regret. As a consequence, ALGnet learns the optimal auction faster than RegretNet while being schedule-free and requiring less hyperparameters.
\end{minipage} 
\hspace*{0.4cm}
\begin{minipage}[h]{0.600\linewidth}
\vspace*{-1.2em}
\begin{table}[H]
\caption{Revenue \& regret of ALGnet for settings (A)-(C). }
\vspace*{-.5em}
\label{fig:table_small_auct}
    \begin{tabular}{lccccccc}
     \toprule
    \multirow{2}{*}{} & 
    \multicolumn{2}{c}{Optimal} & \multicolumn{2}{c}{ALGnet (Ours)}
    \\
    \cmidrule(lr){2-3}
    \cmidrule(lr){4-5}
    & $\mathit{rev}$ & $\mathit{rgt}$ & $\mathit{rev}$ & $\mathit{rgt ~~(\times 10^{-3})}$
    %
    \\
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-3}
    \cmidrule(lr){4-4}
    \cmidrule(lr){5-5}
    (A)
    & $0.550$ & 
    $0$ & 0.555 $(\pm 0.0019)$ & $0.55~(\pm 0.14)$ 
    \\
    % \hline
    (B)
    & 9.781 & 0  & 9.737 $(\pm 0.0443)$ & $0.75~(\pm 0.17)$  
    \\
    % \hline
    
    (C)
    & 0.1706 & $ 0 $& 0.1712 $(\pm 0.0012)$ & $ 0.14~(\pm 0.07)$
    \\ 
    \hline
    \end{tabular}
\end{table}
\end{minipage} 

\vspace{0.2cm}
 
 
 
 
 




\begin{figure}[h]
\vspace{-1em}
\begin{subfigure}{0.33\textwidth}
  \centering
   \includegraphics[width=1.05\linewidth]{images/c1x2Revenue.png}
   \vspace{-2.5em}
  \caption{}
  \label{fig:1}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.05\linewidth]{images/c1x2Regret.png}
  \vspace{-2.5em}
  \caption{}
  \label{fig:2}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.05\linewidth]{images/c1x2P.png} 
  \vspace{-2.5em}
  \caption{}
  \label{fig:3}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.05\linewidth]{images/cRevenueOnline.png}
  \vspace{-2.5em}
  \caption{}
  \label{fig:4}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.05\linewidth]{images/cRegretOnline.png}
  \vspace{-2.5em}
  \caption{}
  \label{fig:5}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.05\linewidth]{images/cPOnline.png}
  \vspace{-2.5em}
  \caption{}
  \label{fig:6}
\end{subfigure}
\vspace{-0.5em}
\caption{(a-b-c) compares the evolution of the revenue, regret and $P^{*}$ as a function of the number of epoch for RegretNet and ALGnet for setting (A).  (d-e-f) plots the the revenue, regret and $P^{*}$ as a function of time for ALGnet and (offline \& online) RegretNet for an online auction (Section~\ref{sec:online}).  } 
\label{fig:comparaisonRegretNet}
\end{figure} 


\paragraph{Unknown and large-scale auctions.} We now consider settings where the optimal auction is unknown. We look at $n$-bidder $m$-item additive settings where the valuations are sampled i.i.d from $\mathcal{U}[0,1]$ which we will denote  by $n \times m$. In addition to "reasonable"-scale auctions ($1\times 10$ and $2\times 2$), we investigate large-scale auctions ($3\times 10$ and $5\times 10$) that are much more complex. Only deep learning methods are able to solve them efficiently.  \autoref{fig:table_large_auct} shows that  ALGnet is able to discover auctions that yield comparable or better results than RegretNet. 



\begin{table}[h]
\caption{Comparison of RegretNet and ALGnet. The values reported for RegretNet are found in \cite{dutting2017optimal}, the numerical values for $\mathit{rgt}$ and standard deviations are not available.
}\label{fig:table_large_auct}

\begin{subfigure}[b]{0.99\textwidth}
\begin{center}
%
%
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{Setting \quad \quad \quad \quad} & 
\multicolumn{2}{c}{RegretNet \quad \quad }& \multicolumn{2}{c}{ALGnet (Ours)}
\\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
& $\mathit{rev}$ & $\mathit{rgt}$ & $\mathit{rev}$ & $\mathit{rgt}$
%
\\
\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-5}
$1 \times 2 $  
& $0.554$ & 
$< 1.0 \cdot 10^{-3}$ & 0.555 $(\pm 0.0019)$ & $0.55 \cdot 10^{-3} (\pm 0.14 \cdot 10^{-3})$ 
\\
% \hline
$1 \times 10 $
& 3.461 & $< 3.0 \cdot 10^{-3}$ & 3.487 $(\pm 0.0135)$ & $1.65 \cdot 10^{-3} (\pm 0.57 \cdot 10^{-3})$  
\\
% \hline

$2 \times 2 $
& 0.878 & $< 1.0 \cdot 10^{-3}$ & 0.879 $(\pm 0.0024)$ & $0.58 \cdot 10^{-3} (\pm 0.23 \cdot 10^{-3})$
\\ 
% \hline

$3 \times 10 $ 
& 5.541 & $<2.0 \cdot 10^{-3}$ & 5.562 $(\pm 0.0308)$ & $ 1.93 \cdot 10^{-3} (\pm 0.33 \cdot 10^{-3})$ 
\\
% \hline

$5 \times 10 $
& 6.778 & $ < 5.0 \cdot 10^{-3}$ & 6.781 $(\pm 0.0504)$ & $3.85 \cdot 10^{-3} (\pm 0.43 \cdot 10^{-3})$\\
\bottomrule
\end{tabular}
\end{center}
\end{subfigure}
\end{table}

\subsection{Online auctions}
\label{sec:online}

 ALGnet is an online algorithm with a time-independent loss function. We would expect it to perform well in settings where the underlying distribution of the valuations  changes over time. We consider a one bidder and  two items additive auction with valuations $v_1$ and $v_2$ sampled i.i.d from $\mathcal{U}[0,1+t]$ where $t$ in increased from $0$ to $1$ at a steady rate. The optimal auction at time $t$ has revenue $0.55\times(1+t)$.
 We use ALGnet and two versions of RegretNet, the original offline version (Appendix A) and our own online version (Appendix B) and plot $\mathit{rev}(t)$, $\mathit{rgt}(t)$ and $P^{*}(t)$ (\autoref{fig:comparaisonRegretNet}). The offline version learns from a fixed dataset of valuations sampled  at $t=0$ (i.e. with $V \sim \mathcal{U}[0,1]^{nm}$) while the online versions (as ALGnet) learns from a stream of data at each time $t$.
 Overall, ALGnet performs better than the other methods. It learns an optimal auction faster at the initial (especially compared to RegretNet Online) and keep adapting to the distributional shift (contrary to vanilla RegretNet).




==> ICLR Auction Game/intro.tex <==
\vspace{-1.1em}
\section{Introduction}
\vspace{-0.6em}
Efficiently designing truthful auctions is a core problem in Mathematical Economics. Concrete examples include the sponsored search auctions conducted by companies as Google or auctions run on platforms as eBay. Following seminal work of Vickrey~\citep{vickrey1961counterspeculation} and Myerson~\citep{myerson1981optimal}, auctions are typically studied in the \emph{independent private valuations} model: each bidder has a valuation function over items, and their payoff depends only on the items they receive. Moreover, the auctioneer knows aggregate information about the population that each bidder comes from, modeled as a distribution over valuation functions, but does not know precisely each bidder's valuation (outside of any information in this Bayesian prior). A major difficulty in designing auctions is that valuations are private and bidders need to be incentivized to report their valuations truthfully.  The goal of the auctioneer is to design an incentive compatible auction which maximizes expected revenue.

\vspace{-0.2em}
Auction Design has existed as a rigorous mathematical field for several decades and yet, complete characterizations of the optimal auction only exist for a few settings. While Myerson's Nobel prize-winning work provides a clean characterization of the single-item optimum \citep{myerson1981optimal}, optimal \emph{multi-item} auctions provably suffer from numerous formal measures of intractability (including computational intractability, high description complexity, non-monotonicity, and others)~\citep{daskalakis2014complexity, ChenDPSY14, ChenDOPSY15, ChenMPY18, HartR15, Thanassoulis04}.

\vspace{-0.2em}
 An orthogonal line of work instead develops deep learning architectures to find the optimal auction.  \cite{dutting2017optimal} initiated this direction by proposing RegretNet, a feed-forward architecture.  They frame the auction design problem as a constrained learning problem and lift the constraints into the objective via the augmented Lagrangian method. Training RegretNet involves optimizing this Lagrangian-penalized objective, while simultaneously updating network parameters and the Lagrangian multipliers themselves. This architecture produces impressive results: recovering near-optimal auctions in several known multi-item settings, and discovering new mechanisms when a theoretical optimum is unknown. %However, the architecture is difficult to train in practice for multiple reasons.
 
 % Non-stationary function optimization  is known to be harder than stationary one [reference].
 
%  Yet, this approach presents several limitations. On the conceptual front, this approach leverages \emph{none} of the vast literature on Auction Theory (other than the optimal auction can be written as a linear program). Our work, on the other hand, leverages an exciting line of recent works~\cite{HartlineL10, HartlineKM11,BeiH11,daskalakis2012symmetries, rubinstein2018simple, DughmiHKN17, CaiOVZ19} 
\vspace{-0.2em}
  Yet, this approach presents several limitations. On the conceptual front, our main insight is a connection to an exciting line of recent works~\citep{HartlineL10, HartlineKM11,BeiH11,daskalakis2012symmetries, rubinstein2018simple, DughmiHKN17, CaiOVZ19} 
 on $\varepsilon$-truthful-to-truthful reductions.\footnote{By $\epsilon$-truthful, we mean the expected total regret $R$ is bounded by  $\epsilon$. See \autoref{prop:main} for a definition of $R$. } On the technical front, we identify three areas for improvement. First, their architecture is difficult to train in practice as the objective is non-stationary. Specifically, the Lagrangian multipliers are time-dependent and they increase following a pre-defined schedule, which requires careful hyperparameter tuning (see~\autoref{subsec:dutt} for experiments illustrating this). Leveraging the aforementioned works in Auction Theory, we propose a \emph{stationary} Lagrangian objective. Second, all prior work inevitably finds auctions which are not \emph{precisely} incentive compatible, and does not provide a metric to compare, say, an auction with revenue $1.01$ which is $0.002$-truthful, or one with revenue $1$ which is $0.001$-truthful. We argue that our stationary Lagrangian objective serves as a good metric (and that the second auction of our short example is ``better'' for our metric). Finally, their training procedure requires an inner-loop optimization (essentially, this inner loop is the bidders trying to maximize utility in the current auction), which is itself computationally expensive. We use amortized optimization to make this process more efficient.

 

 \section*{Contributions}

This paper leverages recent work in Auction Theory to formulate the learning of revenue-optimal auctions as a two-player game. We develop a new algorithm ALGnet (Auction Learning Game network) that produces competitive or better results compared to \cite{dutting2017optimal}'s RegretNet. In addition to the conceptual contributions, our approach yields the following improvements (as RegretNet is already learning near-optimal auctions, our improvement over RegretNet is not due to significantly higher optimal revenues).


\begin{itemize}
    \item[--] \textit{Easier hyper-parameter tuning}: By constructing a time-independent loss function, we circumvent the need to search for an adequate parameter scheduling.  Our formulation also involves less hyperparameters, which makes it more robust.

    \item[--] \textit{A metric to compare auctions}: We propose a metric to compare the quality of two auctions which are not incentive compatible.

    \item[--] \textit{More efficient training}: We replace the inner-loop optimization of prior work with a neural network, which makes training more efficient. 

    \item[--] \textit{Online auctions}: Since the learning formulation is time-invariant, ALGnet is able to quickly adapt in auctions where the bidders' valuation distributions varies over time. Such setting appears for instance in the online posted pricing problem studied in \citet{bubeck2017online}. 
\end{itemize}

 Furthermore, these technical contributions together now imply a novel formulation of auction learning as a two-player game (not zero-sum) between an auctioneer and a misreporter. The auctioneer is trying to design an incentive compatible auction that maximizes revenue while the misreporter is trying to identify breaches in the truthfulness of these auctions. 

The paper decomposes as follows. Section~\ref{sec:setting} introduces the standard notions of auction design. Section~\ref{sec:dutt} presents our game formulation for auction learning. Section~\ref{sec:NN_arch} provides a description of ALGnet and its training procedure. Finally, Section~\ref{sec:exps} presents numerical evidence for the effectiveness of our approach.
 

  

 
 
  

==> ICLR Auction Game/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICLR Auction Game/problem_setup.tex <==
 
\section{Auction design as a time-varying learning problem}\label{sec:setting}

We first review the framework of auction design and the problem of finding truthful mechanisms. We then recall the learning problem proposed by \cite{dutting2017optimal} to find optimal auctions. 

\subsection{Auction design and linear program}

\paragraph{Auction design.} We consider an auction with $n$ bidders and $m$ items. We will denote by $N=\{1,\dots,n\}$ and $M=\{1,\dots,m\}$ the set of bidders and items. Each bidder $i$ values item $j$ at a valuation denoted $v_{ij}$. We will focus on \emph{additive} auctions. These are auctions where the value of a set $S$ of items is equal to the sum of the values of the elements in that set at $\sum_{j \in S} v_{ij}$. Additive auctions are perhaps the most well-studied setting in multi-item auction design~\citep{HartN12, LiY13,daskalakis2014complexity, CaiDW16,daskalakis2017strong}.

The auctioneer does not know the exact valuation profile $V = (v_{ij})_{i\in N, j\in M}$ of the bidders in advance but he does know the distribution from which they are drawn: the valuation vector of bidder $i$, $\vec{v}_i=(v_{i1}, \dots, v_{im})$ is drawn from a distribution $D_i$ over $\mathbb{R}^m$. We will further assume that all bidders are independent and that $D_1 = \cdots = D_n $. As a result V is drawn from $D:= \otimes_{i=1}^n D_i = D_1^{\otimes^n}$.

\begin{definition}
 An auction is defined by a randomized allocation rule $g=(g_1,\dots,g_n)$ and a payment rule $p=(p_1,\dots,p_n)$ where $g_i\colon \mathbb{R}^{n\times m}\rightarrow [0,1]^{m}$ and $p_i\colon \mathbb{R}^{n\times m}\rightarrow \mathbb{R}_{\geq 0}$. Additionally for all items $j$ and valuation profiles $V$, the $g_i$ must satisfy $\sum_i [g_i(V)]_j\leq 1$.
 \end{definition}
 
Given a bid matrix $B=(b_{ij})_{i\in N, j\in M}$, $[g_i(B)]_j$
 is the probability that bidder $i$ receives object $j$ and $p_i(B)$ is the price bidder $i$ has to pay to the auction. The condition $\sum_i [g_i(V)]_j\leq 1$ allows the possibility for an item to be not allocated. 
 
 \begin{definition}
 The utility of bidder $i$ is defined by $u_i(\vec{v}_i,B)= \sum_{j=1}^m [g_i(B)]_j v_{ij} -p_i(B).$ 
\end{definition}

Bidders seek to maximize their utility and may report bids that are different from their true valuations.
In the following, we will denote by $B_{-i}$ the $(n-1)\times m$ bid matrix without bidder $i$, and by $(\vec{b}_i', B_{-i})$ the $n\times m$ bid matrix that inserts $\vec{b}_i'$ into row $i$ of $B_{-i}$ (for example: $B:= (\vec{b}_i, B_{-i})$.
We aim at auctions that incentivize bidders to bid their true valuations.

\begin{definition}\label{def:DSIC}
An auction $(g,p)$ is \textit{dominant strategy incentive compatible} (DSIC) if each bidder's utility is maximized by reporting truthfully no matter what the other bidders report. For every bidder $i,$ valuation $\vec{v}_i \in D_i$, bid $\vec{b}_i\hspace{.02cm}'\in D_i$ and bids $B_{-i}\in D_{-i}$,  $u_i(\vec{v}_i,(\vec{v}_i,B_{-i}))\geq u_i(\vec{v}_i,(\vec{b}_i\hspace{.02cm}',B_{-i})). $ 
\end{definition}
 
\begin{definition}\label{def:IR}
An auction is \textit{individually rational} (IR) if for all $i\in N, \; \vec{v}_i\in D_i$ and $B_{-i}\in D_{-i},$
\begin{equation}\label{eq:IR_eq}\tag{IR}
   u_i(\vec{v}_i,(\vec{v}_i,B_{-i}))\geq 0.  
\end{equation}
\end{definition}

In a DSIC auction, the bidders have the incentive to truthfully report their valuations and therefore, the revenue on valuation profile $V$ is $ \sum_{i=1}^n p_i(V).$ Optimal auction design aims at finding a DSIC and IR auction that maximizes the expected revenue $rev:= \mathbb{E}_{V\sim D}[\sum_{i=1}^n p_i(V)]$.  Since there is no known characterization of DSIC mechanisms in the multi-item setting, we resort to the relaxed notion of \textit{ex-post regret}. It measures the extent to which an auction violates DSIC.


\begin{definition}
The ex-post regret for a bidder $i$ is the maximum increase in his utility when considering all his possible bids and fixing the bids of others. For a valuation profile $V$, it is given by $r_{i}(V)=\max_{\vec{b}_i\hspace{.02cm}'\in \mathbb{R}^m} u_i(\vec{v}_i,(\vec{b}_i\hspace{.02cm}',V_{-i})) - u_i(\vec{v}_i,(\vec{v}_i,V_{-i}))$.  In particular, DSIC is equivalent to 
\begin{equation}\label{eq:regretDSIC}\tag{IC} 
    r_{i}(V)=0, \;  \forall i \in N,  \forall \, V \in D.
\end{equation}
\vspace{-0.2em}
The bid $\vec{b}_i'$ that achieves $r_i(V)$ is called the optimal misreport of bidder $i$ for valuation profile $V$.
\end{definition}
\vspace{-.2cm}
Therefore, finding an optimal auction is equivalent to the following linear program:
\vspace{-.2cm}
\begin{equation*}\tag{LP}\label{eq:exact_prob}
\begin{aligned}
\hspace{-.51cm} \vspace{-1.81cm} \underset{(g,p)\in \mathcal{M} }{\text{min}}
  - \mathbb{E}_{V\sim D}\left[\sum_{i=1}^n p_i(V)\right] \quad \text{s.t.} \quad 
&   r_{i}(V)=0, \hspace{1.55cm} \forall ~i \in N,\;  \forall ~V \in D, \\[-3.5\jot]
& u_i(\vec{v}_i,(\vec{v}_i,B_{-i}))\geq 0, \,\, \forall i\in N,\; \vec{v}_i\in D_i,B_{-i}\in D_{-i}.
\end{aligned}
\end{equation*}

\subsection{Auction design as a learning problem}\label{par:auction}
As the space of auctions $\mathcal{M}$ may be large, we will set a parametric model. In what follows, we consider the class of  auctions $(g^w,p^w)$ encoded by a neural network of parameter $w\in \mathbb{R}^d$.  The corresponding utility and regret function will be denoted by $u_i^w$ and $r_i^w$.

Following \cite{dutting2017optimal}, the formulation  ~\eqref{eq:exact_prob} is relaxed: the IC constraint for all $V\in D$ is replaced by the expected constraint $\mathbb{E}_{V\sim D}[r_i^w(V)]=0$ for all $i\in N.$ The justification for this relaxation can be found in \cite{dutting2017optimal}. By replacing expectations with empirical averages, the learning problem becomes:

 \begin{equation}\label{eq:empirical_prob}\tag{$\widehat{\mathrm{LP}}$}
\begin{aligned}
\underset{w\in \mathbb{R}^d}{\text{min}}
-\frac{1}{L}\sum_{\ell=1}^L \sum_{i=1}^n p_i^w(V^{(\ell)}) \quad \text{s.t.}\quad\widehat{r}_i^w:=\frac{1}{L}\sum_{\ell=1}^L r_i^w(V^{(\ell)})=0,\; \forall i \in N. 
\end{aligned}
\end{equation}
 
The learning problem \eqref{eq:empirical_prob} does not ensure \eqref{eq:IR_eq}. However, this constraint is usually built into the parametrization (architecture) of the model: by design, the only auction mechanism considered satisfy \eqref{eq:IR_eq}.  

Implementation details can be found in  \cite{dutting2017optimal,rahme2020permeq} or in Sec~\ref{sec:NN_arch}.
 


==> ICLR Auction Game/related_work.tex <==

\section*{Related work}

\paragraph{Auction design and machine learning.} Machine learning and computational learning theory have been used in several ways to design auctions from samples of bidder valuations. Machine learning has been used to analyze the sample complexity of designing optimal revenue-maximizing auctions. This includes the framework of single-parameter settings\citep{morgenstern2015pseudo,huang2018making, HartlineT19,RoughgardenS16, GonczarowskiN17, GuoHZ19},  multi-item auctions \citep{dughmi2014sampling, GonczarowskiW18}, combinatorial auctions \citep{balcan2016sample,morgenstern2016learning,syrgkanis2017sample} 
and allocation mechanisms \citep{narasimhan2016general}. Other works have leveraged machine learning to optimize different aspects of mechanisms \citep{lahaie2011kernel,dutting2015payment}. Our approach is different as we build a deep learning architecture for auction design. 

\paragraph{Auction design and deep learning.} While \cite{dutting2017optimal} is the first paper to design auctions through deep learning, several other paper followed-up this work. \cite{feng2018deep} extended it to budget constrained bidders, \cite{golowich2018deep} to the facility location problem. \cite{tacchetti2019neural} built architectures based on the Vickrey-
Clarke-Groves mechanism. \cite{rahme2020permeq} used permutation-equivariant networks to design symmetric auctions.  \cite{shen2019automated} and \cite{dutting2017optimal} proposed architectures that \textit{exactly} satisfy incentive compatibility but are specific to \textit{single-bidder} settings. While all the previously mentioned papers consider a non-stationary objective function, we formulate a time-invariant objective that is easier to train and that makes comparisons between mechanisms possible. 



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

